ABSeeker: Training Long-Horizon Search Agents via Answer-Backtracked Credit Assignment

Long-horizon search agents must make multiple sequential actions (steps) to search, retrieve, verify, and integrate evidence to reach a final answer. However, existing methods for training these agents typically treat all steps within a trajectory uniformly during both supervised fine-tuning (SFT) and reinforcement learning (RL), failing to distinguish useful actions from erroneous or redundant ones. In this paper, we propose Answer-Backtracked Credit Assignment (ABC), a fine-grained credit assignment framework for training long-horizon search agents by converting sparse trajectory-level outcomes into dense step-level supervision that rewards useful actions (even in failed trajectories) while suppressing erroneous or redundant actions. Specifically, given a potentially obscure query and its corresponding ground-truth answer, ABC first performs Answer-Backtracked Clue Recovery, which traces back from the answer to recover intermediate clues required to solve the question. It then applies Clue-Anchored Step Scoring to evaluate each search step against these clues, converting sparse binary outcome supervision into dense step-level rewards. Based on these rewards, we develop ABC-SFT, which reweights the loss of each turn, and ABC-GRPO, which uses the step-level scores as rewards in GRPO. Building on this framework, we train ABSeeker based on Qwen3.5-4B with only 8.5k examples. ABSeeker achieves 37.3% on BrowseComp and 39.1% on BrowseComp-ZH. With context management, the scores further improve to 55.3% and 52.9%, respectively, significantly outperforming same-scale (4B) agents and even matching the performance of larger ones (approximately 30B). These results demonstrate the effectiveness of answer-backtracked step-level credit assignment for training long-horizon search agents.

==> ref_storage.tex <==
\iffalse

@inproceedings{yao2022react,
  title={React: Synergizing reasoning and acting in language models},
  author={Yao, Shunyu and Zhao, Jeffrey and Yu, Dian and Shafran, Izhak and Narasimhan, Karthik R and Cao, Yuan},
  booktitle={NeurIPS 2022 Foundation Models for Decision Making Workshop},
  year={2022}
}

@article{wang2025information,
  title = {Information Gain-based Policy Optimization: A Simple and Effective Approach for Multi-Turn {LLM} Agents},
  author = {Wang, Guoqing and Dai, Sunhao and Ye, Guangze and Gan, Zeyu and Yao, Wei and Deng, Yong and Wu, Xiaofeng and Ying, Zhenzhe},
  year = {2025},
  journal = {arXiv preprint arXiv:2510.14967},
  doi = {10.48550/arXiv.2510.14967}
}

@article{li2026verified,
  title = {Verified Critical Step Optimization for {LLM} Agents},
  author = {Li, Mukai and Zeng, Qingcheng and Fang, Tianqing and Liang, Zhenwen and Song, Linfeng and Liu, Qi and Mi, Haitao and Yu, Dong},
  year = {2026},
  journal = {arXiv preprint arXiv:2602.03412},
  doi = {10.48550/arXiv.2602.03412}
}

@article{liu2026beyond,
  title = {Beyond Trajectory Rewards: Step-level Credit Assignment for Agentic Search via Graph Modeling},
  author = {Liu, Yuchen and Feng, Yingjie and Qin, Lixiong and Chen, Jiasi and Yu, Jianing and Gao, Sheng and Yang, Sheng and Xu, Weiran},
  year = {2026},
  journal = {arXiv preprint arXiv:2605.29697},
  doi = {10.48550/arXiv.2605.29697}
}

@article{li2025websailor,
  title = {{WebSailor}: Navigating Super-human Reasoning for Web Agent},
  author = {Li, Kuan and Zhang, Zhongwang and Yin, Huifeng and Zhang, Liwen and Ou, Litu and Wu, Jialong and Yin, Wenbiao and Li, Baixuan and Tao, Zhengwei and Wang, Xinyu and Shen, Weizhou and Zhang, Junkai and Zhang, Dingchu and Wu, Xixi and Jiang, Yong and Yan, Ming and Xie, Pengjun and Huang, Fei and Zhou, Jingren},
  year = {2025},
  journal = {arXiv preprint arXiv:2507.02592},
  doi = {10.48550/arXiv.2507.02592}
}

@article{du2026openseeker,
  title = {{OpenSeeker}: Democratizing Frontier Search Agents by Fully Open-Sourcing Training Data},
  author = {Du, Yuwen and Ye, Rui and Tang, Shuo and Zhu, Xinyu and Lu, Yijun and Cai, Yuzhu and Chen, Siheng},
  year = {2026},
  journal = {arXiv preprint arXiv:2603.15594},
  doi = {10.48550/arXiv.2603.15594}
}

@article{du2026openseekerv2,
  title = {{OpenSeeker}-v2: Pushing the Limits of Search Agents with Informative and High-Difficulty Trajectories},
  author = {Du, Yuwen and Ye, Rui and Tang, Shuo and Huang, Keduan and Zhu, Xinyu and Cai, Yuzhu and Chen, Siheng},
  year = {2026},
  journal = {arXiv preprint arXiv:2605.04036},
  doi = {10.48550/arXiv.2605.04036}
}

@article{team2025tongyi,
  title={Tongyi deepresearch technical report},
  author={Team, Tongyi DeepResearch and Li, Baixuan and Zhang, Bo and Zhang, Dingchu and Huang, Fei and Li, Guangyu and Chen, Guoxin and Yin, Huifeng and Wu, Jialong and Zhou, Jingren and others},
  journal={arXiv preprint arXiv:2510.24701},
  year={2025}
}

@article{team2026drvenus,
  title = {{DR-Venus}: Towards Frontier Edge-Scale Deep Research Agents with Only 10K Open Data},
  author = {{Venus Team} and Dai, Sunhao and Deng, Yong and Lin, Jinzhen and Song, Yusheng and Wang, Guoqing and Wu, Xiaofeng and Zhou, Yuqi and Yang, Shuo and Ying, Zhenzhe and Zhang, Zhanwei and Meng, Changhua and Wang, Weiqiang},
  year = {2026},
  journal = {arXiv preprint arXiv:2604.19859},
  doi = {10.48550/arXiv.2604.19859}
}

@article{wei2025browsecomp,
  title = {{BrowseComp}: A Simple Yet Challenging Benchmark for Browsing Agents},
  author = {Wei, Jason and Sun, Zhiqing and Papay, Spencer and McKinney, Scott and Han, Jeffrey and Fulford, Isa and Chung, Hyung Won and Passos, Alex Tachard and Fedus, William and Glaese, Amelia},
  year = {2025},
  journal = {arXiv preprint arXiv:2504.12516},
  doi = {10.48550/arXiv.2504.12516}
}

@article{zhou2025browsecompzh,
  title = {{BrowseComp-ZH}: Benchmarking Web Browsing Ability of Large Language Models in Chinese},
  author = {Zhou, Peilin and Leon, Bruce and Ying, Xiang and Zhang, Can and Shao, Yifan and Ye, Qichen and Chong, Dading and Jin, Zhiling and Xie, Chenxuan and Cao, Meng and Gu, Yuxin and Hong, Sixin and Ren, Jing and Chen, Jian and Liu, Chao and Hua, Yining},
  year = {2025},
  journal = {arXiv preprint arXiv:2504.19314},
  doi = {10.48550/arXiv.2504.19314}
}

@article{mialon2023gaia,
  title = {{GAIA}: A Benchmark for General {AI} Assistants},
  author = {Mialon, Gr{\'e}goire and Fourrier, Cl{\'e}mentine and Swift, Craig and Wolf, Thomas and LeCun, Yann and Scialom, Thomas},
  year = {2023},
  journal = {arXiv preprint arXiv:2311.12983},
  doi = {10.48550/arXiv.2311.12983}
}

@article{chen2025xbench,
  title = {xbench: Tracking Agents Productivity Scaling with Profession-Aligned Real-World Evaluations},
  author = {Chen, Kaiyuan and Ren, Yixin and Liu, Yang and Hu, Xiaobo and Tian, Haotong and Xie, Tianbao and Liu, Fangfu and Zhang, Haoye and Liu, Hongzhang and Gong, Yuan and Sun, Chen},
  year = {2025},
  journal = {arXiv preprint arXiv:2506.13651},
  doi = {10.48550/arXiv.2506.13651}
}

@article{xie2026quest,
  title = {{QUEST}: Training Frontier Deep Research Agents with Fully Synthetic Tasks},
  author = {Xie, Jian and Lin, Tianhe and Wang, Zilu and Ning, Yuting and Yao, Yuekun and Xue, Tianci and Zhang, Zhehao and Li, Zhongyang and Zhang, Kai and Wu, Yufan and Chen, Shijie and Gou, Boyu and Han, Mingzhe and Wang, Yifei and Lee, Vint and Wei, Xinpeng and Wang, Xiangjun and Su, Yu and Sun, Huan},
  year = {2026},
  journal = {arXiv preprint arXiv:2605.24218},
  doi = {10.48550/arXiv.2605.24218}
}

@article{gao2025beyond,
  title = {Beyond Ten Turns: Unlocking Long-Horizon Agentic Search with Large-Scale Asynchronous {RL}},
  author = {Gao, Jiaxuan and Fu, Wei and Xie, Minyang and Xu, Shusheng and He, Chuyi and Mei, Zhiyu and Zhu, Banghua and Wu, Yi},
  year = {2025},
  journal = {arXiv preprint arXiv:2508.07976},
  doi = {10.48550/arXiv.2508.07976}
}

@article{shao2024deepseekmath,
  title = {{DeepSeekMath}: Pushing the Limits of Mathematical Reasoning in Open Language Models},
  author = {Zhihong Shao and Peiyi Wang and Qihao Zhu and Runxin Xu and Junxiao Song and Xiao Bi and Haowei Zhang and Mingchuan Zhang and Y.K. Li and Y. Wu and Daya Guo},
  year = {2024},
  journal = {arXiv preprint arXiv:2402.03300},
  doi = {10.48550/arXiv.2402.03300}
}

@misc{openai2025deepresearch,
  title = {Deep Research System Card},
  author = {{OpenAI}},
  year = {2025},
  howpublished = {\url{https://cdn.openai.com/deep-research-system-card.pdf}},
  note = {February 25, 2025}
}

@article{yang2025qwen3,
  title = {{Qwen3} Technical Report},
  author = {Yang, An and Li, Anfeng and Yang, Baosong and Zhang, Beichen and Hui, Binyuan and Zheng, Bo and Yu, Bowen and Gao, Chang and Huang, Chengen and Lv, Chenxu and Zheng, Chujie and Liu, Dayiheng and Zhou, Fan and Huang, Fei and Hu, Feng and Ge, Hao and Wei, Haoran and Lin, Huan and Tang, Jialong and Yang, Jian and Tu, Jianhong and Zhang, Jianwei and Yang, Jianxin and Yang, Jiaxi and Zhou, Jing and Zhou, Jingren and Lin, Junyang and Dang, Kai and Bao, Keqin and Yang, Kexin and Yu, Le and Deng, Lianghao and Li, Mei and Xue, Mingfeng and Li, Mingze and Zhang, Pei and Wang, Peng and Zhu, Qin and Men, Rui and Gao, Ruize and Liu, Shixuan and Luo, Shuang and Li, Tianhao and Tang, Tianyi and Yin, Wenbiao and Ren, Xingzhang and Wang, Xinyu and Zhang, Xinyu and Ren, Xuancheng and Fan, Yang and Su, Yang and Zhang, Yichang and Zhang, Yinger and Wan, Yu and Liu, Yuqiong and Wang, Zekun and Cui, Zeyu and Zhang, Zhenru and Zhou, Zhipeng and Qiu, Zihan},
  year = {2025},
  journal = {arXiv preprint arXiv:2505.09388},
  doi = {10.48550/arXiv.2505.09388}
}

@article{team2026mirothinker,
  title = {{MiroThinker}-1.7 \& {H1}: Towards Heavy-Duty Research Agents via Verification},
  author = {{MiroMind Team} and Bai, S. and Bing, L. and Lei, L. and Li, R. and Li, X. and Lin, X. and Min, E. and Su, L. and Wang, B. and Wang, L. and Wang, S. and Wang, X. and Zhang, Y. and Zhang, Z. and Chen, G. and Chen, L. and Cheng, Z. and Deng, Y. and Huang, Z. and Ng, D. and Ni, J. and Ren, Q. and Tang, X. and Wang, B.L. and Wang, H. and Wang, N. and Wei, C. and Wu, Q. and Xia, J. and Xiao, Y. and Xu, H. and Xu, X. and Xue, C. and Yang, Z. and Ye, F. and Ye, H. and Yu, J. and Zhang, C. and Zhang, W. and Zhao, H. and Zhu, P.},
  year = {2026},
  journal = {arXiv preprint arXiv:2603.15726},
  doi = {10.48550/arXiv.2603.15726}
}

@article{lu2026longseeker,
  title = {{LongSeeker}: Elastic Context Orchestration for Long-Horizon Search Agents},
  author = {Lu, Yijun and Ye, Rui and Du, Yuwen and Wang, Jiajun and Liu, Songhua and Chen, Siheng},
  year = {2026},
  journal = {arXiv preprint arXiv:2605.05191},
  doi = {10.48550/arXiv.2605.05191}
}

@article{team2025mirothinker,
  title = {{MiroThinker}: Pushing the Performance Boundaries of Open-Source Research Agents via Model, Context, and Interactive Scaling},
  author = {{MiroMind Team} and Bai, Song and Bing, Lidong and Chen, Carson and Chen, Guanzheng and Chen, Yuntao and Chen, Zhe and Chen, Ziyi and Dai, Jifeng and Dong, Xuan and Deng, Yue and Fu, Yunjie and Ge, Junqi and Han, Chenxia and Huang, Tammy and Huang, Zhenhang and Jiao, Jerry and Jiang, Shilei and Jiao, Tianyu and Jian, Xiaoqi and Lei, Lei and Li, Ruilin and Luo, Ryan and Li, Tiantong and Lin, Xiang and Liu, Ziyuan and Li, Zhiqi and Ni, Jie and Ren, Qiang and Sun, Pax and Su, Shiqian and Tao, Chenxin and Wang, Bin and Wang, Hellen and Wang, Haonan and Wang, James and Wang, Jin and Wang, Jojo and Wang, Letian and Wang, Shizun and Wang, Weizhi and Wang, Zixuan and Xu, Jinfan and Xing, Sen and Yang, Chenyu and Ye, Hai and Yu, Jiaheng and Yu, Yue and Zhong, Muyan and Zhao, Tianchen and Zhu, Xizhou and Zhou, Yanpeng and Zhang, Yifan and Zhu, Zhi},
  year = {2025},
  journal = {arXiv preprint arXiv:2511.11793},
  doi = {10.48550/arXiv.2511.11793}
}

@article{deepseekai2025deepseekv3,
  title = {{DeepSeek-V3.2}: Pushing the Frontier of Open Large Language Models},
  author = {{DeepSeek-AI} and Liu, Aixin and Mei, Aoxue and Lin, Bangcai and Xue, Bing and Wang, Bingxuan and Xu, Bingzheng and Wu, Bochao and Zhang, Bowei and Lin, Chaofan and Dong, Chen and Lu, Chengda and Zhao, Chenggang and Deng, Chengqi and Xu, Chenhao and Ruan, Chong and Dai, Damai and Guo, Daya and Yang, Dejian and Chen, Deli and Li, Erhang and Zhou, Fangqi and Lin, Fangyun and Dai, Fucong and Hao, Guangbo and Chen, Guanting and Li, Guowei and Zhang, H. and Xu, Hanwei and Li, Hao and Liang, Haofen and Wei, Haoran and Zhang, Haowei and Luo, Haowen and Ji, Haozhe and Ding, Honghui and Tang, Hongxuan and Cao, Huanqi and Gao, Huazuo and Qu, Hui and Zeng, Hui and Huang, Jialiang and Li, Jiashi and Xu, Jiaxin and Hu, Jiewen and Chen, Jingchang and Xiang, Jingting and Yuan, Jingyang and Cheng, Jingyuan and Zhu, Jinhua and Ran, Jun and Jiang, Junguang and Qiu, Junjie and Li, Junlong and Song, Junxiao and Dong, Kai and Gao, Kaige and Guan, Kang and Huang, Kexin and Zhou, Kexing and Huang, Kezhao and Yu, Kuai and Wang, Lean and Zhang, Lecong and Wang, Lei and Zhao, Liang and Yin, Liangsheng and Guo, Lihua and Luo, Lingxiao and Ma, Linwang and Wang, Litong and Zhang, Liyue and Di, M.S. and Xu, M.Y and Zhang, Mingchuan and Zhang, Minghua and Tang, Minghui and Zhou, Mingxu and Huang, Panpan and Cong, Peixin and Wang, Peiyi and Wang, Qiancheng and Zhu, Qihao and Li, Qingyang and Chen, Qinyu and Du, Qiushi and Xu, Ruiling and Ge, Ruiqi and Zhang, Ruisong and Pan, Ruizhe and Wang, Runji and Yin, Runqiu and Xu, Runxin and Shen, Ruomeng and Zhang, Ruoyu and Liu, S.H. and Lu, Shanghao and Zhou, Shangyan and Chen, Shanhuang and Cai, Shaofei},
  year = {2025},
  journal = {arXiv preprint arXiv:2512.02556},
  doi = {10.48550/arXiv.2512.02556}
}

@article{yu2025dapo,
  title = {{DAPO}: An Open-Source {LLM} Reinforcement Learning System at Scale},
  author = {Yu, Qiying and Zhang, Zheng and Zhu, Ruofei and Yuan, Yufeng and Zuo, Xiaochen and Yue, Yu and Fan, Tiantian and Liu, Gaohong and Liu, Lingjun and Liu, Xin and Lin, Haibin and Lin, Zhiqi and Ma, Bole and Sheng, Guangming and Tong, Yuxuan and Zhang, Chi and Zhang, Mofan and Zhang, Wang and Zhu, Hang and Zhu, Jinhua and Chen, Jiaze and Chen, Jiangjie and Wang, Chengyi and Yu, Hongli and Dai, Weinan and Song, Yuxuan and Wei, Xiangpeng and Zhou, Hao and Liu, Jingjing and Ma, Wei-Ying and Zhang, Ya-Qin and Yan, Lin and Qiao, Mu and Wu, Yonghui and Wang, Mingxuan},
  year = {2025},
  journal = {arXiv preprint arXiv:2503.14476},
  doi = {10.48550/arXiv.2503.14476}
}

@article{seed2026seed2,
  title = {{Seed2.0} Model Card: Towards Intelligence Frontier for Real-World Complexity},
  author = {{Bytedance Seed}},
  year = {2026},
  journal = {arXiv preprint arXiv:2607.00248},
  doi = {10.48550/arXiv.2607.00248}
}

@article{miromind2025mirothinker,
  title = {{MiroThinker}: Pushing the Performance Boundaries of Open-Source Research Agents via Model, Context, and Interactive Scaling},
  author = {{MiroMind Team}},
  year = {2025},
  journal = {arXiv preprint arXiv:2511.11793},
  doi = {10.48550/arXiv.2511.11793}
}

@article{jin2025searchr1,
  title = {{Search-R1}: Training {LLMs} to Reason and Leverage Search Engines with Reinforcement Learning},
  author = {Jin, Bowen and Zeng, Hansi and Yue, Zhenrui and Wang, Dong and Zamani, Hamed and Han, Jiawei},
  year = {2025},
  journal = {arXiv preprint arXiv:2503.09516},
  doi = {10.48550/arXiv.2503.09516}
}

@article{song2025r1searcher,
  title = {{R1-Searcher}: Incentivizing the Search Capability in {LLMs} via Reinforcement Learning},
  author = {Song, Huatong and Jiang, Jinhao and Min, Yingqian and Chen, Jie and Chen, Zhipeng and Zhao, Wayne Xin and Fang, Lei and Wen, Ji-Rong},
  year = {2025},
  journal = {arXiv preprint arXiv:2503.05592},
  doi = {10.48550/arXiv.2503.05592}
}

@article{chen2025research,
  title = {{ReSearch}: Learning to Reason with Search for {LLMs} via Reinforcement Learning},
  author = {Chen, Mingyang and Li, Tianpeng and Sun, Haoze and Zhou, Yijie and Zhu, Chenzheng and Yang, Fan and Zhou, Zenan and Chen, Weipeng and Wang, Haofen and Pan, Jeff Z. and Zhang, Wen and Chen, Huajun},
  year = {2025},
  journal = {arXiv preprint arXiv:2503.19470},
  doi = {10.48550/arXiv.2503.19470}
}

@article{zheng2025deepresearcher,
  title = {{DeepResearcher}: Scaling Deep Research via Reinforcement Learning in Real-world Environments},
  author = {Zheng, Yuxiang and Fu, Dayuan and Hu, Xiangkun and Cai, Xiaojie and Ye, Lyumanshan and Lu, Pengrui and Liu, Pengfei},
  year = {2025},
  journal = {arXiv preprint arXiv:2504.03160},
  doi = {10.48550/arXiv.2504.03160}
}

@article{minddr2026minddr,
  title = {{Mind DeepResearch} Technical Report},
  author = {{MindDR Team} and {Li Auto Inc}},
  year = {2026},
  journal = {arXiv preprint arXiv:2604.14518},
  doi = {10.48550/arXiv.2604.14518}
}

@article{zhang2025criticsearch,
  title = {{CriticSearch}: Fine-Grained Credit Assignment for Search Agents via a Retrospective Critic},
  author = {Zhang, Yaocheng and Huang, Haohuan and Song, Zijun and Zhu, Yuanheng and Zhang, Qichao and Zhao, Zijie and Zhao, Dongbin},
  year = {2025},
  journal = {arXiv preprint arXiv:2511.12159},
  doi = {10.48550/arXiv.2511.12159}
}

@article{tang2025deepminer,
  title = {Beyond Turn Limits: Training Deep Search Agents with Dynamic Context Window},
  author = {Tang, Qiaoyu and Xiang, Hao and Yu, Le and Yu, Bowen and Lu, Yaojie and Han, Xianpei and Sun, Le and Zhang, WenJuan and Wang, Pengbo and Liu, Shixuan and Zhang, Zhenru and Tu, Jianhong and Lin, Hongyu and Lin, Junyang},
  year = {2025},
  journal = {arXiv preprint arXiv:2510.08276},
  doi = {10.48550/arXiv.2510.08276}
}

@article{chu2026redsearcher,
  title = {{REDSearcher}: A Scalable and Cost-Efficient Framework for Long-Horizon Search Agents},
  author = {Chu, Zheng and Wang, Xiao and Hong, Jack and Fan, Huiming and Huang, Yuqi and Yang, Yue and Xu, Guohai and Zhao, Chenxiao and Xiang, Cheng and Hu, Shengchao and Kuang, Dongdong and Liu, Ming and Qin, Bing and Yu, Xing},
  year = {2026},
  journal = {arXiv preprint arXiv:2602.14234},
  doi = {10.48550/arXiv.2602.14234}
}

@article{chen2026agentcpmexplore,
  title = {{AgentCPM-Explore}: Realizing Long-Horizon Deep Exploration for Edge-Scale Agents},
  author = {Chen, Haotian and Cong, Xin and Fan, Shengda and Fu, Yuyang and Gong, Ziqin and Lu, Yaxi and Li, Yishan and Niu, Boye and Pan, Chengjun and Song, Zijun and Wang, Huadong and Wu, Yesai and Wu, Yueying and Xie, Zihao and Yan, Yukun and Zhang, Zhong and Lin, Yankai and Liu, Zhiyuan and Sun, Maosong},
  year = {2026},
  journal = {arXiv preprint arXiv:2602.06485},
  doi = {10.48550/arXiv.2602.06485}
}

@misc{openai2025gpt5,
  title = {{OpenAI GPT-5} System Card},
  author = {{OpenAI}},
  year = {2025},
  howpublished = {\url{https://openai.com/index/gpt-5-system-card/}},
}

@misc{google2026gemini31,
  title = {{Gemini 3.1 Pro} Model Card},
  author = {{Google DeepMind}},
  year = {2026},
  howpublished = {\url{https://deepmind.google/models/model-cards/gemini-3-1-pro/}},
}

@article{team2026glm5,
  title = {{GLM-5}: From Vibe Coding to Agentic Engineering},
  author = {{GLM-5 Team} and Zeng, Aohan and Lv, Xin and Hou, Zhenyu and Du, Zhengxiao and Zheng, Qinkai and Chen, Bin and Yin, Da and Ge, Chendi and Xie, Chengxing and Wang, Cunxiang and Pan, Gengzheng and Zeng, Hao and Zhang, Haoke and Wang, Haoran and Chen, Huilong and Zhang, Jiajie and Jiao, Jian and Guo, Jiaqi and Wang, Jingsen and Du, Jingzhao and Wu, Jinzhu and Wang, Kedong and Li, Lei and Fan, Lin and Zhong, Lucen and Liu, Mingdao and Zhao, Mingming and Du, Pengfan and Dong, Qian and Lu, Rui and Li, Shuang and Cao, Shulin and Liu, Song and Jiang, Ting and Chen, Xiaodong and Zhang, Xiaohan and Huang, Xuancheng and Dong, Xuezhen and Xu, Yabo and Wei, Yao and An, Yifan and Niu, Yilin and Zhu, Yitong and Wen, Yuanhao and Cen, Yukuo and Bai, Yushi and Qiao, Zhongpei and Wang, Zihan and Wang, Zikang and Zhu, Zilin and Liu, Ziqiang and Li, Zixuan},
  year = {2026},
  journal = {arXiv preprint arXiv:2602.15763},
  doi = {10.48550/arXiv.2602.15763}
}

@article{deepseekai2026deepseekv4,
  title = {{DeepSeek-V4}: Towards Highly Efficient Million-Token Context Intelligence},
  author = {{DeepSeek-AI}},
  year = {2026},
  journal = {arXiv preprint arXiv:2606.19348},
  doi = {10.48550/arXiv.2606.19348}
}

@misc{anthropic2025claude45,
  title = {{Claude Opus 4.5} System Card},
  author = {{Anthropic}},
  year = {2025},
  howpublished = {\url{https://www.anthropic.com/claude-opus-4-5-system-card}},
}

@misc{zhipu2025glm47,
  title = {{GLM-4.7}: Advancing the Coding Capability},
  author = {{Zhipu AI}},
  year = {2025},
  howpublished = {\url{https://z.ai/blog/glm-4.7}},
}

@article{deepseekv4,
  title   = {{DeepSeek-V4}: Towards Highly Efficient Million-Token Context Intelligence},
  author  = {{DeepSeek-AI}},
  journal = {arXiv preprint arXiv:2606.19348},
  year    = {2026},
  url     = {https://arxiv.org/abs/2606.19348}
}

\fi
